Tangent groupoid and tangent cones in sub-Riemannian geometry

Let $X_1,\cdots,X_m$ be vector fields satisfying H\"ormander's Lie bracket generating condition on a smooth manifold $M$. We generalise Connes's tangent groupoid, by constructing a completion of the space $M\times M\times \mathbb{R}_+^\times$ using the sub-Riemannian metric. We use our space to calculate all the tangent cones of the sub-Riemannian metric in the sense of the Gromov-Hausdorff distance. This generalises a result of Bella\"iche.

==> Packages.tex <==
\usepackage[english]{babel}

%Font issues
\usepackage[T1]{fontenc}%allows one to use pipe sign, less than or equal, etc freely in tex file
\usepackage{lmodern}   
\usepackage{xcolor}%adds colors




%MathTools
\usepackage{amsmath,amsthm,amssymb,amsfonts}%AMS PACKAGE
\usepackage{mathtools}
\usepackage{tensor}%adds \tensor and \indices
\usepackage{tikz-cd}%adds diagrams
\usepackage{esint}%\fint
\usepackage{mathrsfs}%gives fancy mathscr
\usepackage{thmtools}
\usepackage{slashed}
\usepackage{mathabx}

\usepackage{bbm}
\usepackage{microtype}
\usepackage{accents}

%General Structure tools
\usepackage{enumitem}%enumerate package
\usepackage[toc,page]{appendix}%adds appendix
\usepackage{imakeidx}%allows one to maked indices in articles




%Ref Tools
\usepackage{crossreftools}
\usepackage{hyperref}
\usepackage{cleveref}




%General Format
\usepackage{emptypage}%removes numbers from empty pages
\usepackage[a4paper,	bindingoffset=0in,		left=1.2in,		right=1.2in,	top=1in,	bottom=1in,	footskip=.25in]{geometry} %Margin
%\setlength\parindent{5pt}



            
%Bib            
\usepackage[backend=biber,style=alphabetic,sorting=ynt,sortcites]{biblatex}%References
\addbibresource{../../GlobalLibrary.bib}            
            
            
            
%\usepackage{graphicx}%allows pictures \includegraphics{•}
%\usepackage{numprint}%changes numbers format to add a decimal point every three digits etc
%\usepackage{subfiles}%adds subfiles



%Useless
%\usepackage{setspace}

